Learning to Sample with Local and Global Contexts in Experience Replay Buffer

Experience replay, which enables the agents to remember and reuse experience from the past, has played a significant role in the success of off-policy reinforcement learning (RL). To utilize the experience replay efficiently, the existing sampling methods allow selecting out more meaningful experiences by imposing priorities on them based on certain metrics (e.g. TD-error). However, they may result in sampling highly biased, redundant transitions since they compute the sampling rate for each transition independently, without consideration of its importance in relation to other transitions. In this paper, we aim to address the issue by proposing a new learning-based sampling method that can compute the relative importance of transition. To this end, we design a novel permutation-equivariant neural architecture that takes contexts from not only features of each transition (local) but also those of others (global) as inputs. We validate our framework, which we refer to as Neural Experience Replay Sampler (NERS), on multiple benchmark tasks for both continuous and discrete control tasks and show that it can significantly improve the performance of various off-policy RL methods. Further analysis confirms that the improvements of the sample efficiency indeed are due to sampling diverse and meaningful transitions by NERS that considers both local and global contexts.

==> 6_broaderimpact.tex <==
\section*{Broader impact}
% Reinforcement learning (RL) has the potential to be used in a variety of fields, not only artificial inted 

% Reinforcement learning (RL) has proved its broad usages in various domains, not only artificial intelligence, but also robotic-assisted surgery \cite{esteva2019guide}, drug discovery \cite{zhou2019optimization}, and dynamic treatment regimes \cite{yu2019reinforcement}.
This paper focuses on designing a learning-based experience replay in reinforcement learning (RL) which has great potential to outperform humans in a variety of fields, even in robotic-assisted surgery \cite{esteva2019guide}, drug discovery \cite{zhou2019optimization}, and dynamic treatment regimes \cite{yu2019reinforcement}. We believe that our work may contribute to solving some challenges which should be solved to apply RL to the real world.


\textbf{Sample efficiency.} The low sample efficiency is one of fundamental issues in RL to overcome. 
Meanwhile, using a replay buffer has become indispensable in off-policy learning in RL and its sample efficiency largely depends on sampling methods \cite{ddpg_per, deep_q-learning_with_per, sac_boosting}. Accordingly, our work will help improve the efficiency of off-policy RL algorithms, by providing, arguably, a near-optimal solution
about what is the best strategy to utilize the replay buffer.

\textbf{Continual learning.} To apply RL to the real world, it is sometimes required that RL agents should learn when facing a new environment without catastrophic forgetting even if collecting new experience is difficult or expensive, e.g., robotics. It has been revealed that developing a sampling method is one of keys for continual learning \cite{selective_experience, experience_replay_for_continual_learning}. Although our work does not consider this field, we expect that learning-based experience replay may contribute to the improvement of continual learning. 

% \textbf{Learning on environments with sparse rewards.} It is known that one of RL challenges is to deal with sparse rewards. Sparse rewards are  hard to motivate agents to explore and learn in given environments. One of the approaches is to revise replay buffer so that 

% cannot interact with environments.
% in industry or robotics,
% situations arise where gathering new experience is expensive or difficult, and thus simultaneous
% training is infeasible
% RL has the great potential to be used in various fields in the real world, such as robotic-assisted surgery \cite{esteva2019guide}, drug discovery \cite{zhou2019optimization}, and dynamic treatment regimes \cite{yu2019reinforcement}. Indeed, RL agents already showed far superior performance to humans in some tasks \cite{silver2017mastering, vinyals2019grandmaster}. 
% Nevertheless, there are various difficulties in applying RL to the real world \cite{dulac2019challenges} and 
% the low sample efficiency is one of fundamental issues in RL to overcome. 
% Meanwhile, using a replay buffer has become indispensable in off-policy learning in RL and how to use the replay buffer largely affects the sample efficiency. Accordingly, our work will help improve the efficiency of off-policy RL algorithms, by providing, arguably, a near-optimal solution
% about what is the best strategy to utilize the replay buffer.

==> exp_dc.tex <==
\begin{figure}
\begin{centering}
\begin{minipage}[t]{0.333\textwidth}%
\subfigure[Pong (Rainbow)]{\includegraphics[width=1\textwidth]{figures/Pong}\label{fig:pong}} 
\end{minipage}%
\begin{minipage}[t]{0.333\textwidth}%
\subfigure[Freeway (Rainbow)]{\includegraphics[width=1\textwidth]{figures/Freeway}\label{fig:freeway}} 
\end{minipage}%
\begin{minipage}[t]{0.333\textwidth}%
\subfigure[Boxing (Rainbow)]{\includegraphics[width=1\textwidth]{figures/Boxing}\label{fig:boxing}} 
\end{minipage}%
\par\end{centering}
\vspace{-0.1in}
\caption{\label{fig:mainresults-atari} \small Learning curves of Rainbow \cite{van2019use} with various sampling methods on Atari tasks.
The solid line
and shaded regions represent the mean and standard deviation, respectively, across five runs.}
\end{figure}

==> exp_mujoco.tex <==
\begin{figure}
\vspace{-0.4in}
\centering
\begin{centering}
\begin{minipage}[t]{0.32\textwidth}
\subfigure[HalfCheetah (TD3)]{\includegraphics[width=1\textwidth]{figures/HalfCheetah_TD3.png}\label{fig:cheetahtd3}} 
\end{minipage}
\begin{minipage}[t]{0.32\textwidth}
\subfigure[Hopper   (TD3)]{\includegraphics[width=1\textwidth]{figures/Hopper_TD3.png}\label{fig:hoppertd3}}
\end{minipage}%
\begin{minipage}[t]{0.32\textwidth}
\subfigure[IDP  (TD3)]{\includegraphics[width=1\textwidth]{figures/InvertedDoublePendulum_TD3.png}\label{fig:invertd3}}
\end{minipage}%
\par\end{centering}
\vspace{-0.05in}
\begin{centering}
\begin{minipage}[t]{0.32\textwidth}
\subfigure[HalfCheetah  (SAC)]{\includegraphics[width=1\textwidth]{figures/HalfCheetah_SAC.png}\label{fig:cheetahsac}} 
\end{minipage}
\begin{minipage}[t]{0.32\textwidth}
\subfigure[Hopper   (SAC)]{\includegraphics[width=1\textwidth]{figures/Hopper_SAC.png}\label{fig:hoppersac}}
\end{minipage}%
\begin{minipage}[t]{0.32\textwidth}
\subfigure[IDP  (SAC)]{\includegraphics[width=1\textwidth]{figures/InvertedDoublePendulum_SAC.png}\label{fig:inversac}}
\end{minipage}%
\par\end{centering}
\vspace{-0.1in}
\caption{\label{fig:mainresults-mujoco} \small Learning curves of off-policy RL algorithms with various sampling methods on MuJoCo tasks.
The solid line
and shaded regions represent the mean and standard deviation, respectively, across five instances.}
\vspace{-0.1in}
\end{figure}

==> name.tex <==
%%%% ICLR Macros (LaTex)
%%%% Adapted by Hugo Larochelle from the NIPS stylefile Macros
%%%% Style File
%%%% Dec 12, 1990   Rev Aug 14, 1991; Sept, 1995; April, 1997; April, 1999; October 2014

% This file can be used with Latex2e whether running in main mode, or
% 2.09 compatibility mode.
%
% If using main mode, you need to include the commands
%             \documentclass{article}
%             \usepackage{iclr14submit_e,times}
%

% Change the overall width of the page.  If these parameters are
%       changed, they will require corresponding changes in the
%       maketitle section.
%
\usepackage{eso-pic} % used by \AddToShipoutPicture
\RequirePackage{fancyhdr}
\RequirePackage{natbib}

% modification to natbib citations
\setcitestyle{authoryear,round,citesep={;},aysep={,},yysep={;}}

\renewcommand{\topfraction}{0.95}   % let figure take up nearly whole page
\renewcommand{\textfraction}{0.05}  % let figure take up nearly whole page

% Define iclrfinal, set to true if iclrfinalcopy is defined
\newif\ificlrfinal
\iclrfinalfalse
\def\iclrfinalcopy{\iclrfinaltrue}
\font\iclrtenhv  = phvb at 8pt

% Specify the dimensions of each page

\setlength{\paperheight}{11in}
\setlength{\paperwidth}{8.5in}


\oddsidemargin .5in    %   Note \oddsidemargin = \evensidemargin
\evensidemargin .5in
\marginparwidth 0.07 true in
%\marginparwidth 0.75 true in
%\topmargin 0 true pt           % Nominal distance from top of page to top of
%\topmargin 0.125in
\topmargin -0.625in
\addtolength{\headsep}{0.25in}
\textheight 9.0 true in       % Height of text (including footnotes & figures)
\textwidth 5.5 true in        % Width of text line.
\widowpenalty=10000
\clubpenalty=10000

% \thispagestyle{empty}        \pagestyle{empty}
\flushbottom \sloppy

% We're never going to need a table of contents, so just flush it to
% save space --- suggested by drstrip@sandia-2
\def\addcontentsline#1#2#3{}

% Title stuff, taken from deproc.
\def\maketitle{\par
\begingroup
   \def\thefootnote{\fnsymbol{footnote}}
   \def\@makefnmark{\hbox to 0pt{$^{\@thefnmark}$\hss}} % for perfect author
                                                        % name centering
%   The footnote-mark was overlapping the footnote-text,
%   added the following to fix this problem               (MK)
   \long\def\@makefntext##1{\parindent 1em\noindent
                            \hbox to1.8em{\hss $\m@th ^{\@thefnmark}$}##1}
   \@maketitle \@thanks
\endgroup
\setcounter{footnote}{0}
\let\maketitle\relax \let\@maketitle\relax
\gdef\@thanks{}\gdef\@author{}\gdef\@title{}\let\thanks\relax}

% The toptitlebar has been raised to top-justify the first page

\usepackage{fancyhdr}
\pagestyle{fancy}
\fancyhead{}

% Title (includes both anonimized and non-anonimized versions)
\def\@maketitle{\vbox{\hsize\textwidth
%\linewidth\hsize \vskip 0.1in \toptitlebar \centering
{\LARGE\sc \@title\par}
%\bottomtitlebar % \vskip 0.1in %  minus
\ificlrfinal
    \lhead{Published as a conference paper at ICLR 2021}
    \def\And{\end{tabular}\hfil\linebreak[0]\hfil
            \begin{tabular}[t]{l}\bf\rule{\z@}{24pt}\ignorespaces}%
  \def\AND{\end{tabular}\hfil\linebreak[4]\hfil
            \begin{tabular}[t]{l}\bf\rule{\z@}{24pt}\ignorespaces}%
    \begin{tabular}[t]{l}\bf\rule{\z@}{24pt}\@author\end{tabular}%
\else
       \lhead{Under review as a conference paper at ICLR 2021}
   \def\And{\end{tabular}\hfil\linebreak[0]\hfil
            \begin{tabular}[t]{l}\bf\rule{\z@}{24pt}\ignorespaces}%
  \def\AND{\end{tabular}\hfil\linebreak[4]\hfil
            \begin{tabular}[t]{l}\bf\rule{\z@}{24pt}\ignorespaces}%
    \begin{tabular}[t]{l}\bf\rule{\z@}{24pt}Anonymous authors\\Paper under double-blind review\end{tabular}%
\fi
\vskip 0.3in minus 0.1in}}

\renewenvironment{abstract}{\vskip.075in\centerline{\large\sc
Abstract}\vspace{0.5ex}\begin{quote}}{\par\end{quote}\vskip 1ex}

% sections with less space
\def\section{\@startsection {section}{1}{\z@}{-2.0ex plus
    -0.5ex minus -.2ex}{1.5ex plus 0.3ex
minus0.2ex}{\large\sc\raggedright}}

\def\subsection{\@startsection{subsection}{2}{\z@}{-1.8ex plus
-0.5ex minus -.2ex}{0.8ex plus .2ex}{\normalsize\sc\raggedright}}
\def\subsubsection{\@startsection{subsubsection}{3}{\z@}{-1.5ex
plus      -0.5ex minus -.2ex}{0.5ex plus
.2ex}{\normalsize\sc\raggedright}}
\def\paragraph{\@startsection{paragraph}{4}{\z@}{1.5ex plus
0.5ex minus .2ex}{-1em}{\normalsize\bf}}
\def\subparagraph{\@startsection{subparagraph}{5}{\z@}{1.5ex plus
  0.5ex minus .2ex}{-1em}{\normalsize\sc}}
\def\subsubsubsection{\vskip
5pt{\noindent\normalsize\rm\raggedright}}


% Footnotes
\footnotesep 6.65pt %
\skip\footins 9pt plus 4pt minus 2pt
\def\footnoterule{\kern-3pt \hrule width 12pc \kern 2.6pt }
\setcounter{footnote}{0}

% Lists and paragraphs
\parindent 0pt
\topsep 4pt plus 1pt minus 2pt
\partopsep 1pt plus 0.5pt minus 0.5pt
\itemsep 2pt plus 1pt minus 0.5pt
\parsep 2pt plus 1pt minus 0.5pt
\parskip .5pc


%\leftmargin2em
\leftmargin3pc
\leftmargini\leftmargin \leftmarginii 2em
\leftmarginiii 1.5em \leftmarginiv 1.0em \leftmarginv .5em

%\labelsep \labelsep 5pt

\def\@listi{\leftmargin\leftmargini}
\def\@listii{\leftmargin\leftmarginii
   \labelwidth\leftmarginii\advance\labelwidth-\labelsep
   \topsep 2pt plus 1pt minus 0.5pt
   \parsep 1pt plus 0.5pt minus 0.5pt
   \itemsep \parsep}
\def\@listiii{\leftmargin\leftmarginiii
    \labelwidth\leftmarginiii\advance\labelwidth-\labelsep
    \topsep 1pt plus 0.5pt minus 0.5pt
    \parsep \z@ \partopsep 0.5pt plus 0pt minus 0.5pt
    \itemsep \topsep}
\def\@listiv{\leftmargin\leftmarginiv
     \labelwidth\leftmarginiv\advance\labelwidth-\labelsep}
\def\@listv{\leftmargin\leftmarginv
     \labelwidth\leftmarginv\advance\labelwidth-\labelsep}
\def\@listvi{\leftmargin\leftmarginvi
     \labelwidth\leftmarginvi\advance\labelwidth-\labelsep}

\abovedisplayskip 7pt plus2pt minus5pt%
\belowdisplayskip \abovedisplayskip
\abovedisplayshortskip  0pt plus3pt%
\belowdisplayshortskip  4pt plus3pt minus3pt%

% Less leading in most fonts (due to the narrow columns)
% The choices were between 1-pt and 1.5-pt leading
%\def\@normalsize{\@setsize\normalsize{11pt}\xpt\@xpt} % got rid of @ (MK)
\def\normalsize{\@setsize\normalsize{11pt}\xpt\@xpt}
\def\small{\@setsize\small{10pt}\ixpt\@ixpt}
\def\footnotesize{\@setsize\footnotesize{10pt}\ixpt\@ixpt}
\def\scriptsize{\@setsize\scriptsize{8pt}\viipt\@viipt}
\def\tiny{\@setsize\tiny{7pt}\vipt\@vipt}
\def\large{\@setsize\large{14pt}\xiipt\@xiipt}
\def\Large{\@setsize\Large{16pt}\xivpt\@xivpt}
\def\LARGE{\@setsize\LARGE{20pt}\xviipt\@xviipt}
\def\huge{\@setsize\huge{23pt}\xxpt\@xxpt}
\def\Huge{\@setsize\Huge{28pt}\xxvpt\@xxvpt}

\def\toptitlebar{\hrule height4pt\vskip .25in\vskip-\parskip}

\def\bottomtitlebar{\vskip .29in\vskip-\parskip\hrule height1pt\vskip
.09in} %
%Reduced second vskip to compensate for adding the strut in \@author


%% % Vertical Ruler
%% % This code is, largely, from the CVPR 2010 conference style file
%% % ----- define vruler
%% \makeatletter
%% \newbox\iclrrulerbox
%% \newcount\iclrrulercount
%% \newdimen\iclrruleroffset
%% \newdimen\cv@lineheight
%% \newdimen\cv@boxheight
%% \newbox\cv@tmpbox
%% \newcount\cv@refno
%% \newcount\cv@tot
%% % NUMBER with left flushed zeros  \fillzeros[<WIDTH>]<NUMBER>
%% \newcount\cv@tmpc@ \newcount\cv@tmpc
%% \def\fillzeros[#1]#2{\cv@tmpc@=#2\relax\ifnum\cv@tmpc@<0\cv@tmpc@=-\cv@tmpc@\fi
%% \cv@tmpc=1 %
%% \loop\ifnum\cv@tmpc@<10 \else \divide\cv@tmpc@ by 10 \advance\cv@tmpc by 1 \fi
%%    \ifnum\cv@tmpc@=10\relax\cv@tmpc@=11\relax\fi \ifnum\cv@tmpc@>10 \repeat
%% \ifnum#2<0\advance\cv@tmpc1\relax-\fi
%% \loop\ifnum\cv@tmpc<#1\relax0\advance\cv@tmpc1\relax\fi \ifnum\cv@tmpc<#1 \repeat
%% \cv@tmpc@=#2\relax\ifnum\cv@tmpc@<0\cv@tmpc@=-\cv@tmpc@\fi \relax\the\cv@tmpc@}%
%% % \makevruler[<SCALE>][<INITIAL_COUNT>][<STEP>][<DIGITS>][<HEIGHT>]
%% \def\makevruler[#1][#2][#3][#4][#5]{\begingroup\offinterlineskip
%% \textheight=#5\vbadness=10000\vfuzz=120ex\overfullrule=0pt%
%% \global\setbox\iclrrulerbox=\vbox to \textheight{%
%% {\parskip=0pt\hfuzz=150em\cv@boxheight=\textheight
%% \cv@lineheight=#1\global\iclrrulercount=#2%
%% \cv@tot\cv@boxheight\divide\cv@tot\cv@lineheight\advance\cv@tot2%
%% \cv@refno1\vskip-\cv@lineheight\vskip1ex%
%% \loop\setbox\cv@tmpbox=\hbox to0cm{{\iclrtenhv\hfil\fillzeros[#4]\iclrrulercount}}%
%% \ht\cv@tmpbox\cv@lineheight\dp\cv@tmpbox0pt\box\cv@tmpbox\break
%% \advance\cv@refno1\global\advance\iclrrulercount#3\relax
%% \ifnum\cv@refno<\cv@tot\repeat}}\endgroup}%
%% \makeatother
%% % ----- end of vruler

%% % \makevruler[<SCALE>][<INITIAL_COUNT>][<STEP>][<DIGITS>][<HEIGHT>]
%% \def\iclrruler#1{\makevruler[12pt][#1][1][3][0.993\textheight]\usebox{\iclrrulerbox}}
%% \AddToShipoutPicture{%
%% \ificlrfinal\else
%% \iclrruleroffset=\textheight
%% \advance\iclrruleroffset by -3.7pt
%%   \color[rgb]{.7,.7,.7}
%%   \AtTextUpperLeft{%
%%     \put(\LenToUnit{-35pt},\LenToUnit{-\iclrruleroffset}){%left ruler
%%       \iclrruler{\iclrrulercount}}
%%   }
%% \fi
%% }
%%% To add a vertical bar on the side
%\AddToShipoutPicture{
%\AtTextLowerLeft{
%\hspace*{-1.8cm}
%\colorbox[rgb]{0.7,0.7,0.7}{\small \parbox[b][\textheight]{0.1cm}{}}}
%}

